High Energy Neutrino Telescopes

This paper presents a review of the history, motivation and current status of high energy neutrino telescopes. Many years after these detectors were first conceived, the operation of kilometer-cubed scale detectors is finally on the horizon at both the South Pole and in the Mediterranean Sea. These new detectors will perhaps provide us the first view of high energy astrophysical objects with a new messenger particle and provide us with our first real glimpse of the distant universe at energies above those accessible by gamma-ray instruments. Some of the topics that can be addressed by these new instruments include the origin of cosmic rays, the nature of dark matter, and the mechanisms at work in high energy astrophysical objects such as gamma-ray bursts, active galactic nuclei, pulsar wind nebula and supernova remnants.

==> debug_log_11515 <==

#####Fri Dec 19 09:47:02 2008#####
STARTED admin_astro-ph.karahoffman.2804


#####Fri Dec 19 09:47:02 2008#####
------------------------------------------------------------------------------
\\
arXiv:0812.3798
From: Kara Hoffman <kara@umd.edu>
Date: Thu, 18 Dec 2008 21:57:08 GMT   (000kb)

Title: High Energy Neutrino Telescopes
Authors: K.D. Hoffman
Categories: astro-ph
Comments: 33 pages, 21 figures, accepted for publication in the New Journal of
  Physics
License: http://arxiv.org/licenses/nonexclusive-distrib/1.0/
Policy: accept
Upload-archive: astro-ph
Upload-subject: hput admin_astro-ph.karahoffman.2804
archive: astro-ph
is-an-author: 1
\\
  This paper presents a review of the history, motivation and current status of
high energy neutrino telescopes. Many years after these detectors were first
conceived, the operation of kilometer-cubed scale detectors is finally on the
horizon at both the South Pole and in the Mediterranean Sea. These new
detectors will perhaps provide us the first view of high energy astrophysical
objects with a new messenger particle and provide us with our first real
glimpse of the distant universe at energies above those accessible by gamma-ray
instruments. Some of the topics that can be addressed by these new instruments
include the origin of cosmic rays, the nature of dark matter, and the
mechanisms at work in high energy astrophysical objects such as gamma-ray
bursts, active galactic nuclei, pulsar wind nebula and supernova remnants.
\\


#warnings_now: ADMIN UPLOAD



#author_warnings_now: 
Author 1: K.D. Hoffman



#####Fri Dec 19 09:47:03 2008#####
Finished unpacking (errors=)

#warnings_now: ADMIN UPLOAD

HENT_rev3.tex did not end with \n, TRUNCATED?


#author_warnings_now: 
Author 1: K.D. Hoffman

 9999151.tar: unpacked 33 files from tar file
 astro-ph.karahoffman.2804.tar: unpacked 33 files from tar file


#####Fri Dec 19 09:47:03 2008#####
showtime: 0812.3798 being processed as test/9999151 -> /data/ftp/arxiv/papers/0812


#####Fri Dec 19 09:47:03 2008#####
packing to 0812.3798.tar.gz

#####Fri Dec 19 09:47:04 2008#####
running AutoTeX -p test/9999151 -d 0812.3798 at Fri Dec 19 09:47:04 2008

#####Fri Dec 19 09:47:05 2008#####
completed AutoTeX in 1s

#####Fri Dec 19 09:47:05 2008#####
Rejected after unpack_submission()... cleaning up

#warnings_now: ADMIN UPLOAD

HENT_rev3.tex did not end with \n, TRUNCATED?
Fri Dec 19 09:47:05 2008: AutoTeX took 1s


#####Fri Dec 19 09:47:05 2008#####
About to close and move this log to /u0/incoming/admin_astro-ph.karahoffman.2804 which will then be moved to /u0/incoming/rejects


==> debug_log_9167 <==

#####Fri Dec 19 09:42:54 2008#####
STARTED admin_astro-ph.karahoffman.2804


#####Fri Dec 19 09:42:54 2008#####
------------------------------------------------------------------------------
\\
arXiv:0812.3798
From: Kara Hoffman <kara@umd.edu>
Date: Thu, 18 Dec 2008 21:57:08 GMT   (000kb)

Title: High Energy Neutrino Telescopes
Authors: K.D. Hoffman
Categories: astro-ph
Comments: 33 pages, 21 figures, accepted for publication in the New Journal of
  Physics
License: http://arxiv.org/licenses/nonexclusive-distrib/1.0/
Policy: accept
Upload-archive: astro-ph
Upload-subject: hput admin_astro-ph.karahoffman.2804
archive: astro-ph
is-an-author: 1
\\
  This paper presents a review of the history, motivation and current status of
high energy neutrino telescopes. Many years after these detectors were first
conceived, the operation of kilometer-cubed scale detectors is finally on the
horizon at both the South Pole and in the Mediterranean Sea. These new
detectors will perhaps provide us the first view of high energy astrophysical
objects with a new messenger particle and provide us with our first real
glimpse of the distant universe at energies above those accessible by gamma-ray
instruments. Some of the topics that can be addressed by these new instruments
include the origin of cosmic rays, the nature of dark matter, and the
mechanisms at work in high energy astrophysical objects such as gamma-ray
bursts, active galactic nuclei, pulsar wind nebula and supernova remnants.
\\


#warnings_now: ADMIN UPLOAD



#author_warnings_now: 
Author 1: K.D. Hoffman



#####Fri Dec 19 09:42:54 2008#####
Finished unpacking (errors=)

#warnings_now: ADMIN UPLOAD

HENT_rev3.tex did not end with \n, TRUNCATED?


#author_warnings_now: 
Author 1: K.D. Hoffman

 astro-ph.karahoffman.2804.tar: unpacked 33 files from tar file


#####Fri Dec 19 09:42:54 2008#####
showtime: 0812.3798 being processed as test/9999151 -> /data/ftp/arxiv/papers/0812


#####Fri Dec 19 09:42:54 2008#####
packing to 0812.3798.tar.gz

#####Fri Dec 19 09:42:55 2008#####
running AutoTeX -p test/9999151 -d 0812.3798 at Fri Dec 19 09:42:55 2008

#####Fri Dec 19 09:42:56 2008#####
completed AutoTeX in 1s

#####Fri Dec 19 09:42:56 2008#####
Rejected after unpack_submission()... cleaning up

#warnings_now: ADMIN UPLOAD

HENT_rev3.tex did not end with \n, TRUNCATED?
Fri Dec 19 09:42:56 2008: AutoTeX took 1s


#####Fri Dec 19 09:42:56 2008#####
About to close and move this log to /u0/incoming/admin_astro-ph.karahoffman.2804 which will then be moved to /u0/incoming/rejects

